Load Balancing for MapReduce-based Entity Resolution

The effectiveness and scalability of MapReduce-based implementations of complex data-intensive tasks depend on an even redistribution of data between map and reduce tasks. In the presence of skewed data, sophisticated redistribution approaches thus become necessary to achieve load balancing among all reduce tasks to be executed in parallel. For the complex problem of entity resolution, we propose and evaluate two approaches for such skew handling and load balancing. The approaches support blocking techniques to reduce the search space of entity resolution, utilize a preprocessing MapReduce job to analyze the data distribution, and distribute the entities of large blocks among multiple reduce tasks. The evaluation on a real cloud infrastructure shows the value and effectiveness of the proposed load balancing approaches.

==> related.tex <==
\section{Related Work}
\label{sec:related}

Load balancing and skew handling are well-known data management problems and MR has been criticized for having overlooked the skew issue \cite{MRCritics}. Parallel database systems already implement skew handling mechanisms, e.g., for parallel hash join processing \cite{DBLP:conf/vldb/DeWittNSS92} that share many similarities with our problem.


A theoretical analysis of skew effects for MR is given in~\cite{Lin2009mapred} but focuses on linear processing of entities in the reduce phase. It disregards the N-squared complexity of comparing all entities with each other. \cite{Kwon:2010:SPP:1807128.1807140} reports that the \mysf{reduce} runtime for scientific tasks does not only depend on the assigned workload (e.g., number of pairs) but also on the data to process. The authors propose a framework for automatic extraction of signatures for (spatial) data to reduce the computational skew. This approach is orthogonal to ours: it addresses computational skew and does not consider effective handling of present data skew.



A fairness-aware key partitioning approach for MR that targets locality-aware scheduling of reduce tasks is proposed in \cite{DBLP:conf/cloudcom/IbrahimJLWHQ10}. The key idea is to assign \mysf{map} output to reduce tasks that eventually run on nodes that already hold a major part of the corresponding data. This is achieved by a modification of the MR framework implementation to control the scheduling of reduce tasks. Similar to our BDM, this approach determines the key distribution to optimize the partitioning. However, it does not split large blocks but still processes all data sharing the same key at the same reduce task which may lead to unbalanced reduce workloads.  



% They argue that data transfer during the repartitioning of data between the map and reduce phase becomes a time critical factor and target locality-aware scheduling of reduce tasks. Therefore, they basically try to assign map output keys (ordered by descending frequency) to reduce tasks that run on nodes that hold a major part of the corresponding data. This approach has several drawbacks. First of all, values having the same key are still assigned to the same reduce task. Due to the quadratic complexity of the comparison of all values with the same key in \mysf{reduce}, the execution time of this reduce task will still dominate the overall execution time although some network traffic might be saved. From our experience, the time for processing the input data and repartitioning data is comparatively negligible to the execution time of reduce tasks given a large dataset and pairwise comparison of all entities sharing the same signature. We therefore proposed two strategies that are capable to deal with extremely skewed data by splitting up reduce tasks into several smaller tasks while still guaranteeing that all values with the same key are compared. As we do, the authors of \cite{DBLP:conf/cloudcom/IbrahimJLWHQ10} count the frequencies of intermediate keys after the map phase and repartition data based on this metadata. However, their approach requires to change the MapReduce framework because firstly a master nodes needs to aggregate the metadata produced by the map tasks and secondly the initialization of reduce tasks is deferred until the metadata is evaluated because the skew handling is realized between the map and reduce phase. We in turn avoid this by aggregating signature frequencies in the reduce phase of a first job and implementing the load balancing in the map phase of a subsequently executed job (see Figure~\ref{fig:overview}). 


MR has already been employed for ER (e.g., \cite{wang_mapdupreducer}) but we are only aware of one load balancing mechanism for MR-based ER. \cite{springerlink:10.1007/s00450-011-0177-x} studies load balancing for Sorted Neighborhood (SN). However, SN follows a different blocking approach that is by design less vulnerable to skewed data.

MR's inherent vulnerability to data skew is relevant for all kind of pairwise similarity computation. Example applications include pairwise document similarity \cite{DBLP:conf/acl/ElsayedLO08} to identify similar documents, set-similarity joins \cite{DBLP:conf/sigmod/VernicaCL10} for efficient string similarity computation in databases, pairwise distance computation \cite{Qiu:2009:CTB:1646468.1646474} for clustering complex objects, and all-pairs matrix computation \cite{DBLP:journals/tpds/MorettiBHRFT10} for scientific computing. All approaches follow a similar idea like ER using blocking: One or more signatures (e.g., tokens or terms) are generated per object (e.g., document) to avoid the computation of the Cartesian product. MR groups together objects sharing (at least) one signature and performs similarity computation within the reduce phase. Simple approaches like \cite{DBLP:conf/acl/ElsayedLO08} create many signatures per object which leads to unnecessary computation because similar objects are likely to have more than one signature in common and are thus compared multiple times. Advanced approaches such as \cite{DBLP:conf/sigmod/VernicaCL10} reduce unnecessary computation by employing filters (e.g., based on token frequencies) that still guarantee that similar object pairs share at least one signature.


A more general case is the computation of theta-joins with MapReduce \cite{DBLP:conf/sigmod/OkcanR11}. Static load balancing mechanisms are not suitable due to arbitray join condititions. Similar to our approach \cite{DBLP:conf/sigmod/OkcanR11} employs a pre-analysis phase to determine the datasets' characteristics (using sampling) and thereby avoids the evaluation of the Cartesian product. This approach is more coarse-grained when compared to our strategies. 


% \textcolor{red}{ER can be regarded as Theta-Joins. \cite{DBLP:conf/sigmod/OkcanR11} proposes a randomized algorithm for the evaluation of arbitrary join conditions on the Cartesian product of two input sources. Naturally, the evaluation of the Cartesian product is less susceptible to skew effects. Furthermore given a input size dominated join problem (as ER is), we found that randomizing the distribution of data items to reduce tasks leads suboptimal execution times and unrepeatable experiments and therefore propose to utilize a Round-robin-like scheduling. Additionally, the authors present a sampling-based optimization to extract the datasets' characteristics and to avoid the evaluation of the Cartesian product. However, this pruning of comparisons is still to coarse-grained applied to our scenario.}





Load balancing is only one aspect towards an optimal execution of MR programs. For example, Manimal \cite{DBLP:conf/webdb/CafarellaR10} employs static code analysis to optimize MR programs. Hadoop++ \cite{DBLP:journals/pvldb/DittrichQJKSS10} proposes index and join techniques that are realized using appropriate partitioning and grouping functions, amongst others.
 



% An interesting skew handling approach for distributed reasoning over RDF datasets was presented in~\cite{DBLP:conf/www/KotoulasOH10}. Instead of a statical assignment of data to compute units they propose to assign data items to a dynamically-stretching region of compute units based on their key. In regions data is randomly exchanged whereas data items with the same key that are located at the same place are processed. However, this and similar approaches cannot be realized with MR due to the MR-inherent principle of static key partitioning.

% Load balancing and skew handling is a well-known problem in parallel database systems. A skew handling algorithm for parallel hash join processing (what shares many similarities with our problem) is discussed in \cite{DBLP:conf/vldb/DeWittNSS92}. As \mysf{Block Split} and \mysf{PairRange} the algorithm relies on key range partitioning, replication of single entities to multiple processors (reduce tasks) and virtual processor partitioning ($r=k\cdot \hat r$). Their load balancing approach relies on sampling instead of a full parallel input scan. However, since matching two entities is clearly computationally more expensive than the comparison of two join attribute values, we argue that the scanning overhead is acceptable and leave sampling-based load balancing for future work.

==> summary_outlook.tex <==
\section{Summary and outlook}
\label{sec:summary}

We proposed two load balancing approaches, \mysf{BlockSplit} and \mysf{PairRange}, for parallelizing blocking-based entity resolution using the widely available MapReduce framework. Both approaches are capable to deal with skewed data (blocking key) distributions and effectively distribute the workload among all reduce tasks by splitting large blocks. Our evaluation in a real cloud environment using real-world data demonstrated that both approaches are robust against data skew and scale with the number of available nodes. The \mysf{BlockSplit} approach is conceptionally simpler than \mysf{PairRange} but achieves already excellent results. \mysf{PairRange} is less dependent on the initial partitioning of the input data and slightly more scalable for large match tasks. 

In future work, we will extend our approaches to multi-pass blocking that assigns multiple blocks per entity. We will further investigate how our load balancing approaches can be adapted for MapReduce-based implementations of other data-intensive tasks, such as join processing or data mining.

% \vspace{\baselineskip} \noindent
% {\bf Acknowledgments:} \\ This work was supported by an Amazon Web Service (AWS) in Education research grant.
 

